A Formal, Resource Consumption-Preserving Translation of Actors to Haskell

We present a formal translation of an actor-based language with cooperative scheduling to the functional language Haskell. The translation is proven correct with respect to a formal semantics of the source language and a high-level operational semantics of the target, i.e. a subset of Haskell. The main correctness theorem is expressed in terms of a simulation relation between the operational semantics of actor programs and their translation. This allows us to then prove that the resource consumption is preserved over this translation, as we establish an equivalence of the cost of the original and Haskell-translated execution traces.

==> highlevel_semantics.tex <==
\section{Enrique}

% \subsection{Notation}

% \paragraph{Substitutions}~\\
% 
% Substitutions are denoted by $\tau$. The substitution $[x \mapsto e]$ replaces the varible $x$ by $e$. Substitution application is juxtaposition, e.g., if $t=x+1+(x-2)$ and $\tau = [x \mapsto e]$ then $t\tau = e+1+(e-2)$.
% 
% \paragraph{Heap modifiers}
% \begin{itemize}
%  \item $h[count \mapsto count + 1]$ generates a heap equal to $h$ but with the counter incremented
%  \item $h[k \mapsto \bot]$ generates a heap equal to $h$ but with the future variable $k$ set to $\bot$
%  \item $h[(n,x) \mapsto v]$ generates a heap equal to $h$ but with the field variable $x$ of object $o$ set to $v$
%  \item Heap modifiers can be chained: $h[count \mapsto count+1, k \mapsto \bot, (n,x) \mapsto v]$
% \end{itemize}
% 
% I use the same notation in Haskell, suppose that it is translated into \texttt{lookup}, \texttt{insert}, etc. functions.

% % \paragraph{Eval functions}~\\
% % \begin{equation*}
% % eval(v,o,h) = \left\{
% % \begin{array}{rl}
% % v & \text{~~~if } v \in \mi{Refs}\\
% % h(o)(v) & \text{~~~if } v \in \mi{Var}\\
% % \end{array} \right.
% % \end{equation*}
% % 
% % \begin{equation*}
% % eval_H(v,o_n,h) = \left\{
% % \begin{array}{rl}
% % r & \text{~~~if } v = \texttt{Param}~r\\
% % \texttt{lookup}~h~o_n~y & \text{~~~if } v = \texttt{Attr}~y\\
% % \end{array} \right.
% % \end{equation*}



% \subsection{ABS operational semantics}\label{sec:op_semantics}
% 
% \subsubsection{Local rules}
% 
% $$
% \inference[(\textsc{Assign I})]
% {
% h' = h[ (n)(x) \mapsto h(n)(y)] 
% }
% {
% \langle n: (\texttt{x:=y};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Assign II})]
% {
% h' = h[ (n)(x) \mapsto r] 
% }
% {
% \langle n: (\texttt{x:=r};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{New})]
% {
% h(\mi{count}) = m & h' = h[ (n)(x) \mapsto m, (m) \mapsto \epsilon, \mi{count} \mapsto m + 1] 
% }
% {
% \langle n: (\texttt{x:=new};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Get})]
% {
% h(h(n)(f)) \neq \bot & h' = h[(n)(x) \mapsto h(h(n)(f))] \\
% }
% {
% \langle n: (\texttt{x:=f.get};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Await I})]
% {
% h(h(n)(f)) \neq \bot \\
% }
% {
% \langle n: (\texttt{await f};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Await II})]
% {
% h(h(n)(f)) = \bot \\
% }
% {
% \langle n: (\texttt{await f};S,l) \cdot Q, h \rangle \rightarrow \langle n: Q \cdot (\texttt{await f};S,l), h \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Async})]
% {
% h(n)(x) = d & h(\mi{count}) = l & \bar{r} = h(n)(\bar{z}) \\
% h' = h[(n)(f) \mapsto l, (l) \mapsto \bot,\mi{count} \mapsto l+1]
% }
% {
% \langle n: (\texttt{f:=x!m($\bar{z}$)};S,l) \cdot Q, h \rangle \stackrel{d.m(l,\bar{r})}{\longrightarrow} \langle n: (S,l) \cdot Q, h' \rangle
% }
% $$
% 
% 
% 
% $$
% \inference[(\textsc{Sync})]
% {
% (m(\bar{w}) \mapsto S_m) \in D~\mathit{fresh} & \tau = [\bar{w} \mapsto h(n)(\bar{z})] & S' = \widehat{(S_m\tau)}^x
% % (m(\bar{w}) \mapsto S_m) \in D~\mathit{fresh} & \tau = [\bar{w} \mapsto eval(\bar{z},n,h)] & S' = \widehat{(S_m\tau)}^x
% }
% {
% \langle n: (\texttt{x:=m($\bar{z}$)};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S';S,l) \cdot Q, h \rangle
% }
% $$
% 
% I suppose that synchronous methods $m$ have only one \texttt{return} statement, and it is the final instruction of its body. $\widehat{*}^x$ is defined as:
% 
% \begin{equation*}
% \widehat{S}^x = \left\{
% \begin{array}{rl}
% \widehat{S_1}^x;\widehat{S_2}^x & \text{~~~if } S=S_1;S_2,\\
% \texttt{x:=z} & \text{~~~if } S=\texttt{return z},\\
% S & \text{~~~i.o.c}.
% \end{array} \right.
% \end{equation*}
% 
% $$
% \inference[(\textsc{Return})]
% {
% h' = h[(l) \mapsto h(n)(x)]
% }
% {
% \langle n: (\texttt{return x};S,l) \cdot Q, h \rangle \rightarrow \langle n: Q, h' \rangle
% }
% $$
% 
% \subsubsection{Global rules}
% 
% $$
% \inference[(\textsc{Internal})]
% {
% \langle n: Q, h \rangle \to \langle n: Q', h' \rangle
% }
% {
% \langle (n:Q) \cup C, h \rangle \rightarrow \langle (n: Q') \cup C, h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Message})]
% {
% \langle n: Q_n, h \rangle \stackrel{d.m(l,\bar{r})}{\longrightarrow} \langle n: Q', h' \rangle & m(\bar{w}) \mapsto S \in D & \tau = [\bar{w} \mapsto \bar{r}]
% }
% {
% \langle (n:Q_n) \cup (d:Q_d) \cup C, h \rangle \rightarrow \langle (n: Q') \cup (d:Q_d\cdot(S\tau,l)) \cup C, h' \rangle
% }
% $$

\subsection{High-level Haskell AST semantics}
Haskell configurations are $\mi{(Heap,SchedQ)}$, where:
\begin{itemize}
 \item $\mi{Heap}$ ``maps'' object references to local heaps and process queues. To retrieve the value of variable $x$ in object $n$ we use the notation $h(n)(x)$. To retrieve the process queue of object $n$ we use the special $\procq$: $h(n)(\procq) = (k,l):q$, where $k$ is a continuation, $l$ the destiny future variable and $q$ the rest of the process queue.
 \item $\mi{SchedQ} = [\overline{o_m}]$ is a queue of object references.
\end{itemize}

We consider a function $\nextO{Heap}{SchedQ}$ that returns the first object in \emph{SchedQ} whose first process is not blocked. We use $[\overline{o_m}]$ to denote the queue/list $[o_1,o_2,\ldots,o_m]$, and $[\overline{o_{i\to k}}]$ for the subqueue/sublist $[o_i,o_{i+i},\ldots,o_k]$ if $k \geq i$. If $k < i$ then $[\overline{o_{i\to k}}] = \epsilon$, the empty queue.

We also consider functions $\newQadd$ and $\newQdel$ defined as:
\begin{equation*}
\newQadd([\overline{o_m}],o_n,o_y) = \left\{
\begin{array}{rl}
[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}] & \text{~~~if } o_y \in [\overline{o_m}] \\
~[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}]:o_y & \text{~~~if } o_y \notin [\overline{o_m}]\\
\end{array} \right.
\end{equation*}

\begin{equation*}
\newQdel([\overline{o_m}],o_n,q_y) = \left\{
\begin{array}{rl}
[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n-1}}] & \text{~~~if } q_n = \epsilon \\
~[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}] & \text{~~~if } q_n \neq \epsilon \\
\end{array} \right.
\end{equation*}



% $$
% \inference[(\textsc{Assign I})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Assign}~x~(\texttt{Attr}~y)~k' \\
% h' = h[ (o_n)(x) \mapsto h(o_n)(y), (o_n)(\procq) \mapsto (k',l):q]\\
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% }
% $$
% 
% $$
% \inference[(\textsc{Assign II})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Assign}~x~(\texttt{Param}~r)~k' \\
% h' = h[ (o_n)(x) \mapsto r, (o_n)(\procq) \mapsto (k',l):q]\\
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% }
% $$
% 
% $$
% \inference[(\textsc{New})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Assign}~x~\texttt{New}~k' & h(count)= o_{new}\\
% % Sched' = \texttt{fromList}~\redt{(o_m,[~])}:[\ldots , (o_n, (k',l):q), \ldots] \\
% %Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] \\
% h' = h[ (o_n)(x) \mapsto o_{new}, count \mapsto o_{new}+1, \\%(o_{new}) \mapsto \epsilon, \\ 
% (o_{new})(\procq) \mapsto \epsilon, (o_n)(\procq) \mapsto (k',l):q]}
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% %\langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Async})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q & h(count) = l'\\
% k(\emptyset) = \texttt{Assign}~x~(\texttt{Async}~y~m~\bar{z})~k' & h(o_n)(y) = o_y & h(o_y)(\procq) = q_y \\
% (m(\bar{w}) \mapsto S) \in D & k'' = \texttt{m}(h(o_n)(\bar{z}),o_n,\texttt{Nothing},\redt{\lambda~\emptyset
%  \to \texttt{undefined}}) \\
% %\tau = [\bar{w} \mapsto h(o_n)(\bar{z})] & \\
% %Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots,(o_m, q_m:(k'',l')),\ldots] \\
% \newQadd([\overline{o_m}],o_n,o_y) = s\\
%  h' = h[ (o_n)(x) \mapsto l', count \mapsto l'+1, l' \mapsto \bot, \\
%  (o_n)(\procq) \mapsto (k',l):q, (o_y)(\procq) \mapsto q_y:(k'',l')]
% }
% {
% (h,[\overline{o_m}]) \toH (h',s)
% % \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots,(o_m, q_m),\ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% %\redt{Similar if $o_n = o_m$, but appending the task into the same queue $q$}
% 
% $$
% \inference[(\textsc{Sync})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Assign}~x~(\texttt{Sync}~m~\bar{z})~k' & (m(\bar{w}) \mapsto S) \in D \\
% k'' = \texttt{m}(h(o_n)(\bar{z}),o_n,\texttt{Just}~x,\redt{k'}) \\
% h' = h[(o_n)(\procq) \mapsto (k'',l):q]
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% %\langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h \rangle
% }
% $$
% Every method $m$ has a Haskell function $\texttt{m} :: [Ref] \to \mi{ObjRef} \to \mi{Maybe~String} \to Cont \to Stmt$ that generates the continuation to execute the method followed by the the passed continuation. The instructions are substituted using the value of the parameters and the last \text{return} statement is decorated to know if the final value must be stored in some field or in a future.
% 
% The continuation returned by \texttt{m} must verify the following property: it creates exactly the same instructions that the method $m$ contains. To state that we use a translation $t$ from statements to ABS instructions:
% 
% $$
% \begin{array}{r@{~=~}l}
% t(\texttt{Assign}~x~(\texttt{Attr~y})~\_) & \texttt{x:=y}\\
% t(\texttt{Assign}~x~(\texttt{Param~r})~\_) & \texttt{x:=r}\\
% t(\texttt{Assign}~x~(\texttt{New})~\_) & \texttt{x:=new}\\
% t(\texttt{Assign}~x~(\texttt{Get}~y)~\_) & \texttt{x:=y.get}\\
% t(\texttt{Assign}~x~(\texttt{Async}~y~m~\bar{z})~\_) & \texttt{x:=y!m($\bar{z}$)}\\
% t(\texttt{Assign}~x~(\texttt{Sync}~m~\bar{z})~\_) & \texttt{x:=m($\bar{z}$)}\\
% t(\texttt{Skip}~\_) & \texttt{skip}\\
% t(\texttt{Return}~x~\texttt{Nothing}~\_) & \texttt{return~x}\\
% t(\texttt{Return}~z~(\texttt{Just~}x)~\_) & \texttt{x:=z}\\
% \end{array}
% $$
% 
% \textbf{Property:} If $(m(\bar{w}) \mapsto S) \in D$ fresh, $\tau = [\bar{w} \mapsto \bar{p}, \this \mapsto o_n]$, $S\tau = b_1;b_2;\ldots;b_n$, $\texttt{m}(\bar{p},o_n,\texttt{Nothing},k') = k$ and
% \begin{itemize}
%  \item $k(\emptyset) = s_1~k_1$
%  \item $k_1(\emptyset) = s_2~k_2$
%  \item[] ~~~~~~~~~\vdots
%  \item $k_{n-1}(\emptyset) = s_n~k_n$
%  %\item $k_{n}(\emptyset) = \texttt{Stop}$
% \end{itemize}
% then $b_i = t(s_i~k_i)$ and $k' = k_n$, where $s~k$ represents an arbitrary statement with continuation $k$.
% 
% The same for synchronous methods, but in this case $\widehat{S\tau}^x = b_1;b_2;\ldots;b_n$, and $\texttt{m}(\bar{p},o_n,(\texttt{Just}~x),k') = s_1~k_1$.

% $$
% \inference[(\textsc{Get})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Assign}~x~(\texttt{Get}~f)~k' & h(h(o_n)(f)) = \texttt{Just}~v \\
% h' = h[ (o_n)(x) \mapsto v, (o_n)(\procq) \mapsto (k',l):q]
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% }
% $$
% 
% $$
% \inference[(\textsc{Await I})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Await}~f~k' & h(h(o_n)(f)) = \texttt{Just}~v \\
% h' = h[(o_n)(\procq) \mapsto (k',l):q]\\
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% }
% $$
% 
% $$
% \inference[(\textsc{Await II})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Await}~f~k' & h(h(o_n)(f)) = \texttt{Nothing} \\
% h' = h[(o_n)(\procq) \mapsto q:(k,l)]\\
% %Sched' = \texttt{fromList}~[\ldots , (o_n, q:(\lambda~\emptyset \to \texttt{Await}~f~k',l)), \ldots] \\
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% }
% $$
% 
% $$
% \inference[(\textsc{Return$_A$})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Return}~z~\texttt{Nothing}~\_ & \newQdel([\overline{o_m}],o_n,q) = s\\
% h' = h[l \mapsto h(o_n)(z), (o_n)(\procq) \mapsto q] \\
% % ~\\
% % Sched' = \texttt{fromList}~[\ldots , (o_n, q), \ldots] & h' = h[l \mapsto h(o_n)(z)]\\
% }
% {
% (h,[\overline{o_m}]) \toH (h',s)
% }
% $$
% 
% % \redt{We may need an additional rule when returning from the last task, to remove the entry of $o_n$ from $Sched'$}
% 
% $$
% \inference[(\textsc{Return$_S$})]
% {
% \nextO{h}{[\overline{o_m}]} = o_n & h(o_n)(\procq) = (k,l):q \\
% k(\emptyset) = \texttt{Return}~z~(\texttt{Just~x})~k'\\
%  & h' = h[(o_n)(x) \mapsto h(o_n)(z),
% (o_n)(\procq) \mapsto (k',l):q]\\
% }
% {
% (h,[\overline{o_m}]) \toH (h',[\overline{o_{n+1\to m}}]:[\overline{o_{1\to n}}])
% }
% $$

% \subsection{Relating ABS operational semantics to \cite{AlbertACGGPR15}}
% 
% The language in Section~\ref{sec:lang} and the semantics in Section~\ref{sec:op_semantics} are a simplified version of those in \emph{Object-Sensitive Cost Analysis for Concurrent Objects}, Albert et al.~\cite{AlbertACGGPR15}. The main differences are:
% \begin{itemize}
%  \item the representation of the states
%  \item the syntax of method invocations (both synchronous and asynchronous),
%  \item in~\cite{AlbertACGGPR15} they consider local variables and class declarations
% \end{itemize}
% 
% 
% In~\cite{AlbertACGGPR15} states are sets of futures and objects, which contain their queues of pending tasks. Formally an object is represented as $ob(o,C,h,\langle tv,\bar{b}\rangle,\mathcal{Q})$, where $o$ is the \emph{object identifier}, $C$ is the \emph{class}, $h$ is the \emph{object heap}, $tv$ is the \emph{table of local variables}, $\bar{b}$ is the sequence of instructions to execute, and $\mathcal{Q}$ the \emph{set of pending tasks}. Futures are represented as $fut(fn,v)$, where $f$ is the future identifier and $v$ its value, possibly $\bot$. The operational semantics in~\cite{AlbertACGGPR15} rewrites states $S \leadsto S'$.
% 
% We will consider a slight variation of the operational semantics in~\cite{AlbertACGGPR15} where fields can be directly assigned by \texttt{new} and \texttt{get} instructions, arbitrary expression in the right-handd side, and future variables can be fields instead of local variables. This modification does not affect the upper bounds and the results obtained in~\cite{AlbertACGGPR15}.
% 
% \begin{definition}[Translation of states]\label{def:translateABS_COSTA}~\\
% $objs(C)$ returns the set of object identifiers in the set $C$.\\
% $futs(h)$ returns the set of future variables in the heap $h$.
% 
% $$
% \begin{array}{rcl}
% \tr{ \langle C, h \rangle }_c & = & \{ ob(n,\_,h(n),a,t) | (n:Q) \in C, (a,t) =  \tr{Q}_q \} \cup \\
%                            &   &\{ ob(o,\_,\epsilon,\epsilon,\emptyset) | o \in Dom(h) \smallsetminus objs(C) \} \cup \\
%                            &   & \{ fut(fn,v) | fn \in futs(h), h(fn) = v \}\\[.3cm]
% \tr{\epsilon}_q & = & (\epsilon,\emptyset)\\
% \tr{(S;l) \cdot (S_1;l_1) \cdot \ldots \cdot (S_n;l_n)}_q & = & (\langle [\texttt{ret} \mapsto l], \tr{S}_s\rangle, \\
%  & & \{ \langle [\texttt{ret} \mapsto l_1], \tr{S_1}_s\rangle, \ldots, \langle [\texttt{ret} \mapsto l_n], \tr{S_n}_s\rangle\}\\[.3cm]
%  
% \tr{\epsilon}_s & = & \epsilon\\
% \tr{\texttt{x:=y};S}_s & = & \texttt{this.x:=this.y};\tr{S}_s\\
% \tr{\texttt{x:=r};S}_s & = & \texttt{this.x:=r};\tr{S}_s\\
% \tr{\texttt{x:=new};S}_s & = & \texttt{this.x:=new C};\tr{S}_s\\
% \tr{\texttt{x:=f.get};S}_s & = & \texttt{this.x:=f.get};\tr{S}_s\\
% \tr{\texttt{f:=x!p($\bar{z}$)};S}_s & = & \texttt{call(m,p(x,$\bar{z}$,f))};\tr{S}_s\\
% \tr{\texttt{f:=p($\bar{z}$)};S}_s & = & \texttt{call(b,p(this,$\bar{z}$,\_))};\tr{S}_s\\
% \tr{\texttt{await f};S}_s & = & \texttt{await f?};\tr{S}_s\\
% \tr{\texttt{return x};S}_s & = & \texttt{return x};\tr{S}_s\\
% \end{array}
% $$
% \end{definition}
% 
% 
% \begin{theorem}\label{teo:ABS_COSTA_steps}
%  If $\langle C, h \rangle \todec{n}{b} \langle C', h' \rangle$ then:
%  \begin{itemize}
%   \item $ \tr{\langle C, h \rangle}_c \leadstodec{n}{\tr{b}_s} \tr{\langle C', h' \rangle}_c$ or,
%   \item $ \tr{\langle C, h \rangle}_c \leadstodec{n}{\tr{b}_s} S \leadstodec{n}{\epsilon} \tr{\langle C', h' \rangle}_c$
%  \end{itemize}
% \end{theorem}
% 
% \redt{In some cases it needs 2 $\leadsto$-steps because of the rule that selects the next task. Our ABS semantics simply takes the next in the queue automatically.}
% \begin{proof}
%  By case distinction on the derivation applied to perform the $\to$-step.
%  \begin{itemize}
%  
%   \item \textbf{\textsc{(Internal)+(Assign I)}}.
%   $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
% % \langle n: Q, h \rangle \to \langle n: Q', h' \rangle
% \inference[\textsc{\tiny{(Assign I)}}]
% {
% h' = h[ (n)(x) \mapsto h(n)(y)] 
% }
% {
% \langle n: (\texttt{x:=y};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h' \rangle
% }
% }
% {
% S_1 \equiv \langle (n:(\texttt{x:=y};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{x:=y}} \langle (n: (S,l) \cdot Q) \cup C, h' \rangle \equiv S_2
% }
% $$
% The translation of $S_1$ is 
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{this.x:=this.y};\tr{S}_s\rangle,Q_{tr}) | R\}$$
% where $R$ is the rest of objects and future variables not involved in the step and $Q_{tr}$ the translation of $Q$. From $\tr{S_1}_c$ it is possible to perform a $\leadsto$-step using rule (2) in~\cite{AlbertACGGPR15}, reaching $\tr{S_2}_c$:
% $$
% \inference[(2)]
% {
% v = h(n)(y)
% }
% {
% \begin{array}{l}
%  \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{this.x:=this.y};\tr{S}_s\rangle,Q_{tr}) | R \} \leadstodec{n}{\texttt{this.x:=this.y}} \\
% \{ ob(n,\_,h(n)[x \mapsto v],\langle [\texttt{ret}\mapsto l], \tr{S}_s\rangle,Q_{tr}) | R \} \equiv \tr{S_2}_c
% \end{array}
% }
% $$
% 
% \item \textbf{\textsc{(Internal)+(Assign II)}}. Similar to the \textsc{(Internal)+(Assign I)} case.
% 
% \item \textbf{\textsc{(Internal)+(New)}}.
% $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
% \inference[\tiny{(\textsc{New})}]
% {
% h(\mi{count}) = m \\ h' = h[ (n)(x) \mapsto m, (m) \mapsto \epsilon, \mi{count} \mapsto m + 1] 
% }
% {
% \langle n: (\texttt{x:=new};S,l) \cdot Q, h \rangle \to \langle n: (S,l) \cdot Q, h' \rangle
% }
% }
% {
% S_1 \equiv \langle (n:(\texttt{x:=new};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{x:=new}} \langle (n: (S,l) \cdot Q) \cup C, h' \rangle \equiv S_2
% }
% $$
% The translation of $S_1$ is 
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{this.x:=new};\tr{S}_s\rangle,Q_{tr}) | R \}$$
% From $\tr{S_1}_c$ it is possible to perform a $\leadsto$-step using rule (3) in~\cite{AlbertACGGPR15}, reaching $\tr{S_2}_c$:
% $$
% \inference[(3)]
% {m = newRef() & newHeap(\_,\epsilon)}
% {\begin{array}{l}
% \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{this.x:=new};\tr{S}_s\rangle,Q_{tr}) | R \} \leadstodec{n}{\texttt{this.x:=new}} \\ 
% \{ ob(n,\_,h(n)[x \mapsto m],\langle [\texttt{ret}\mapsto l], \tr{S}_s\rangle,Q_{tr}), 
% \{ ob(m,\_,\epsilon,\epsilon,\emptyset)| R \} = \tr{S_2}_c
%  \end{array}
% }
% $$
% Note that $m$ is a new object reference as it has been generated using the counter, and the heap
% of the new object generated by $newHeap$ is $\epsilon$ because we do not consider class declarations. No object with identifier $m$ appears in $C$ of $S_2$, but it is generated by the translation because $m$ is in the domain of $h$ (second set of $\tr{\cdot}_c$)
% 
% \item \textbf{\textsc{(Internal)+(Get)}}.
% $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
% \inference[\tiny{(\textsc{Get})}]
% {
% h(h(n)(f)) \neq \bot & h' = h[(n)(x) \mapsto h(h(n)(f))] \\
% }
% {
% \langle n: (\texttt{x:=f.get};S,l) \cdot Q, h \rangle \to \langle n: (S,l) \cdot Q, h' \rangle
% }
% }
% {
% \begin{array}{ll}
% S_1 \equiv \langle (n:(\texttt{x:=f.get};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{x:=f.get}} \\
% \langle (n: (S,l) \cdot Q) \cup C, h' \rangle \equiv S_2 
% \end{array}
% }
% $$
% 
% The translation of $S_1$ is:
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{this.x:=f.get};\tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \}$$
% 
% From $\tr{S_1}_c$ it is possible to perform a $\leadsto$-step using rule (8) in~\cite{AlbertACGGPR15}:
% $$
% \inference[(8)]
% {h(n)(f) = \mi{fn} & v \neq \bot}
% {\begin{array}{l}
% \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{this.x:=f.get};\tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \} \leadstodec{n}{\texttt{this.x:=f.get}} \\ 
% \{ ob(n,\_,h(n)[x \mapsto v],\langle [\texttt{ret}\mapsto l], \tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \} = \tr{S_2}_c
%  \end{array}
% }
% $$
% Note that by the definition of the translation $\tr{\cdot}_c$ we have that $h(h(n)(f)) = v$
% 
% \item \textbf{\textsc{(Internal)+(Await I)}}.
% $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
% \inference[\tiny{(\textsc{Await I})}]
% {
% h(h(n)(f)) \neq \bot  \\
% }
% {
% \langle n: (\texttt{await f};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S,l) \cdot Q, h \rangle
% }
% }
% {
% \begin{array}{ll}
% S_1 \equiv \langle (n:(\texttt{await f};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{await f}} \\
% \langle (n: (S,l) \cdot Q) \cup C, h \rangle \equiv S_2 
% \end{array}
% }
% $$
% 
% The translation of $S_1$ is:
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \}$$
% 
% From $\tr{S_1}_c$ it is possible to perform a $\leadsto$-step using rule (9) in~\cite{AlbertACGGPR15}:
% $$
% \inference[(9)]
% {h(h(n)(f)) \neq \bot}
% {\begin{array}{l}
% \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \} \leadstodec{n}{\texttt{await f?}} \\ 
% \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \} = \tr{S_2}_c
%  \end{array}
% }
% $$
% Note that by the definition of the translation $\tr{\cdot}_c$ we have that $h(n)(f) = \mi{fn}$
% 
% \item \textbf{\textsc{(Internal)+(Await II)}}. This case is similar to the previous one but involving 2 $\leadsto$-steps: one that evaluates the \texttt{await f} that cannot continue and releases the object, and one that schedules the next task in the object.
% 
% $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
% \inference[\tiny{(\textsc{Await II})}]
% {
% h(h(n)(f)) = \bot  \\
% }
% {
% \langle n: (\texttt{await f};S,l) \cdot Q, h \rangle \rightarrow \langle n: Q\cdot((\texttt{await f};S,l)), h \rangle
% }
% }
% {
% \begin{array}{ll}
% S_1 \equiv \langle (n:(\texttt{await f};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{await f}} \\
% \langle (n: Q\cdot((\texttt{await f};S,l))) \cup C, h \rangle \equiv S_2 
% \end{array}
% }
% $$
% 
% Consider that $\tr{Q\cdot((\texttt{await f};S,l))}_q = (a,t)$, where $a$ is the translation of the first task in the queue and $t$ the translation of the rest of the queue. The translation of $S_1$ is:
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \}$$
% 
% From $\tr{S_1}_c$ we can perform a $\leadsto$-step using rule (10) in~\cite{AlbertACGGPR15}:
% $$
% \inference[(10)]
% {h(h(n)(f)) = \bot}
% {\begin{array}{l}
% \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle,Q_{tr}), \mi{fut(fn,v)} | R \} \leadstodec{n}{\texttt{await f?}} \\ 
% \{ ob(n,\_,h(n),\epsilon,\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle \cup Q_{tr}), \mi{fut(fn,v)} | R \} = S'
%  \end{array}
% }
% $$
% Similar to the previous case, we know that $h(n)(f) = \mi{fn}$. From the state $S'$ we can apply rule (11) to schedule a task in the queue $\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle \cup Q_{tr}$, which is the same queue $a \cup t$. Rule (11) can schedule task $a$, performing the $\leadsto$-step:
% $$
% \inference[(11)]
% {a \in \langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle \cup Q_{tr}}
% {\begin{array}{l}
% \{ ob(n,\_,h(n),\epsilon,\langle [\texttt{ret}\mapsto l], \texttt{await f?};\tr{S}_s\rangle \cup Q_{tr}), \mi{fut(fn,v)} | R \} \leadstodec{n}{\epsilon} \\ 
% \{ ob(n,\_,h(n),a,t), \mi{fut(fn,v)} | R \} = \tr{S_2}_c
%  \end{array}
% }
% $$
% 
% Therefore we have the two-step $\leadsto$-derivation $\tr{S_1}_c \leadstodec{n}{\texttt{await f?}} S' \leadstodec{n}{\epsilon} \tr{S_2}_c$.
% 
% 
% \item \textbf{\textsc{(Internal)+(Sync)}}.
%  $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
%   \inference[\textsc{\tiny{(Sync)}}]
%   {
%   (m(\bar{w}) \mapsto S_m) \in D~\mathit{fresh} & \tau = [\bar{w} \mapsto h(n)(\bar{z})] & S' = \widehat{(S_m\tau)}^x
%   }
%   {
%   \langle n: (\texttt{x:=m($\bar{z}$)};S,l) \cdot Q, h \rangle \rightarrow \langle n: (S';S,l) \cdot Q, h \rangle
%   }
% }
% {
% S_1 \equiv \langle (n:(\texttt{x:=m($\bar{z}$)};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{x:=m($\bar{z}$)}} \langle (n: (S';S,l) \cdot Q) \cup C, h \rangle \equiv S_2
% }
% $$
% The translation of $S_1$ is 
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l],\texttt{call(b,m(this,$\bar{z}$,\_))};\tr{S}_s\rangle,Q_{tr}) | R\}$$
% where $R$ is the rest of objects and future variables not involved in the step and $Q_{tr}$ the translation of $Q$. From $\tr{S_1}_c$ it is possible to perform a $\leadsto$-step using rule (4) in~\cite{AlbertACGGPR15}, reaching $\tr{S_2}_c$:
% $$
% \inference[(4)]
% {
% (m(\bar{w}) \mapsto S_m) \in \tr{D}_{sync}^x~\mathit{fresh} & \tau = [\bar{w} \mapsto h(n)(\bar{z})] 
% }
% {
% \begin{array}{l}
%  \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l],\texttt{call(b,m(this,$\bar{z}$,\_))};\tr{S}_s\rangle,Q_{tr}) | R\} \leadstodec{n}{\texttt{call(b,m(this,$\bar{z}$,\_))}} \\
% \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l], S_m\tau;\tr{S}_s\rangle,Q_{tr}) | R \} \equiv \tr{S_2}_c
% \end{array}
% }
% $$
% $\tr{D}_{sync}^x$ is the translation of all the methods in the program $D$ where methods are treated synchronously, i.e., they store a final value in the field $x$. We consider a simplification of the operational semantics in~\cite{AlbertACGGPR15} where synchronous methods return exactly one value, thus the last instruction of a synchronous method stores the final value in the corresponding field. In this case it is easy to check that $\tr{\widehat{(S_m\tau)}^x} = S_m\tau$.
% 
% \item \textbf{\textsc{(Internal)+(Return)}}.
% $$
% \inference[\textsc{\tiny{(Internal)}}]
% {
%   \inference[(\textsc{Return})]
%   {
%   h' = h[(l) \mapsto h(n)(x)]
%   }
%   {
%   \langle n: (\texttt{return x};S,l) \cdot Q, h \rangle \rightarrow \langle n: Q, h' \rangle
%   }
% }
% {
% S_1 \equiv \langle (n:(\texttt{return x};S,l) \cdot Q) \cup C, h \rangle \todec{n}{\texttt{return x}} \langle (n: (S,l) \cdot Q) \cup C, h' \rangle \equiv S_2
% }
% $$
% The translation of $S_1$ is 
% $$\tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l],\texttt{return x};\tr{S}_s\rangle,Q_{tr}), \mi{fut}(l,\bot) | R\}$$
% where $R$ is the rest of objects and future variables not involved in the step and $Q_{tr}$ the translation of $Q$. From $\tr{S_1}_c$ it is possible to perform a $\leadsto$-step using rule (7) in~\cite{AlbertACGGPR15}:
% $$
% \inference[(7)]
% {
% %\texttt{ret} \in dom([\texttt{ret}\mapsto l]) & 
% v = h(n)(x)
% }
% {
% \begin{array}{l}
%  \tr{S_1}_c = \{ ob(n,\_,h(n),\langle [\texttt{ret}\mapsto l],\texttt{return x};\tr{S}_s\rangle,Q_{tr}), \mi{fut}(l,\bot) | R\} \leadstodec{n}{\texttt{return x}} \\
% \{ ob(n,\_,h(n),\epsilon,Q_{tr}), \mi{fut}(l,v) | R\} = S'
% \end{array}
% }
% $$
% If empty -> finished
% 
% Otherwise -> Consider that $\tr{Q}_c = (a,t)$, so $Q_{tr} = a \cup t$. Then we can apply rule (11) to schedule the task $a$ in 
% 
% \item \textbf{\textsc{(Message)+(Async)}}.
%  \end{itemize}
% 
% \end{proof}
% 
% \begin{lemma}[Correspondence of traces]\label{teo:traces}
%  Consider a trace $\langle C_1, h_1 \rangle \to^{b_1} \langle C_2, h_2 \rangle \to^{b_2} \ldots \to^{b_n} \langle C_n, h_n \rangle$ where each step is decorated with the executed instruction $b_i$. Then $\langle \tr{C_1, h_1 \rangle}_c \leadsto^{\tr{b_1}_s} \tr{\langle C_2, h_2 \rangle}_c \leadsto^{\tr{b_2}_s} \ldots \leadsto^{\tr{b_n}_s} \tr{\langle C_n, h_n \rangle}_c$
% \end{lemma}





% \subsection{High-level Haskell semantics \redt{(OLD VERSION!)}}
% 
% $$
% \inference[(\textsc{Assign I})]
% {
% k(h) = \texttt{Yield}~h'~k'~\texttt{x:=y} & h' = h[ (o_n)(x) \mapsto h(o_n)(y)]\\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] \\
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Assign II})]
% {
% k(h) = \texttt{Yield}~h'~k'~\texttt{x:=r} & h' = h[ (o_n)(x) \mapsto r]\\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] \\
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{New})]
% {
% k(h) = \texttt{Yield}~h'~k'~\texttt{x:=new} & h(count)= o_m\\
% Sched' = \texttt{fromList}~(o_m,[~]):[\ldots , (o_n, (k',l):q), \ldots] \\
% h' = h[ (o_n)(x) \mapsto o_m, count \mapsto o_m+1, \redt{(o_m)(this) \mapsto o_m}]}
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Async})]
% {
% k(h) = \texttt{Yield}~h'~k'~\texttt{x:=y!m($\bar{z}$)} & h(o_n)(y) = o_m & h(count) = l\\
% (m(\bar{w}) \mapsto S) \in D & k' = \lambda h_1 \rightarrow m(h'(o_n)(\bar{z}),h_1,\redt{id}) \\
% %\tau = [\bar{w} \mapsto h(o_n)(\bar{z})] & \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots,(o_m, q_m:(k',l)),\ldots] \\
% h' = h[ (o_n)(x) \mapsto l, count \mapsto l+1, l \mapsto \bot]
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots,(o_m, q_m),\ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Sync})]
% {
% k(h) = \texttt{Yield}~h~k'~\redt{k_c}~\texttt{x:=m($\bar{z}$)} \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] & k' = \lambda h_1 \to m(h(o_n)(\bar{z}),h,k_c)
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h \rangle
% }
% $$
% I suppose that for every synchronous method $m$ we have a Haskell function $m :: \mi{Mark \to Refs \to Heap \to Cont \to Pausable}$ invoked as $m(mark,\bar{r},h,k_c)$ that generates a new continuation from $k_c$ (the code after the synchronous call) appending the continuation from the code of $m$. The instructions in \texttt{Yield} terms will contain the $mark$, that will be unique.
% 
% The continuation generated by $m$ must verify the following property: execute exactly the same instructions that the method contains. Let $(m(\bar{w}) \mapsto b^\star_1;b^\star_2;\ldots b^\star_r;) \in^\star D$ a method in the program. Instructions $b^\star_i$ have the ``mark'' $\star$ that is unique, to distinguish between instructions generated by other method invocations.
% 
% $
% \forall k \in Cont. \forall \mi{params}. \forall h \in Heap. \forall Sched~\textnormal{containing the continuation}~\lambda h \to m(\star,\mi{params},h,k)~\textnormal{somewhere in the queue of object}~\hat{o}.\\
% IF~T = \langle Sched,h \rangle \to_{o_1}^{b_1} \langle Sched_1,h_1 \rangle \to_{o_2}^{b_2} \ldots \to_{o_n}^{b_n} \langle Sched_n,h_n \rangle\\
% THEN~T|_{(\hat{o},\star)}~\textnormal{~is a~prefix~of}~b^\star_1;b^\star_2;\ldots b^\star_r;
% $
% 
% Where $T|_{(o,\star)}$ is the sequence of instructions executed in the trace $T$ considering only those in the object $o$ and marked with $\star$.
% 
% $$
% \inference[(\textsc{Get})]
% {
% k(h) = \texttt{Yield}~h'~k'~\texttt{x:=f.get} & h(h(o_n)(f)) \neq \bot \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] \\
% h' = h[ (o_n)(x) \mapsto h(h(o_n)(f))]
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Await I})]
% {
% k(h) = \texttt{Yield}~h~k'~\texttt{await f} & h(h(o_n)(f)) \neq \bot \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] \\
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Await II})]
% {
% k(h) = \texttt{Yield}~h~k'~\texttt{await f} & h(h(o_n)(f)) = \bot \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, q:(k',l)), \ldots] \\
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Return I})]
% {
% k(h) = \texttt{Stop}~h'~k'~(\texttt{Async}~\redt{l})~\texttt{return z} \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, q), \ldots] & h' = h[l \mapsto h(o_n)(z)]\\
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
% 
% $$
% \inference[(\textsc{Return II})]
% {
% k(h) = \texttt{Stop}~h'~k'~(\texttt{Sync}~x)~\texttt{return z} \\
% Sched' = \texttt{fromList}~[\ldots , (o_n, (k',l):q), \ldots] & h' = h[(o_n)(x) \mapsto h(o_n)(z)]\\
% }
% {
% \langle \texttt{fromList}~[\ldots , (o_n, (k,l):q), \ldots], h \rangle \rightarrow \langle Sched', h' \rangle
% }
% $$
